First-Order Model Checking on Structurally Sparse Graph Classes

A class of graphs is structurally nowhere dense if it can be constructed from a nowhere dense class by a first-order transduction. Structurally nowhere dense classes vastly generalize nowhere dense classes and constitute important examples of monadically stable classes. We show that the first-order model checking problem is fixed-parameter tractable on every structurally nowhere dense class of graphs. Our result builds on a recently developed game-theoretic characterization of monadically stable graph classes. As a second key ingredient of independent interest, we provide a polynomial-time algorithm for approximating weak neighborhood covers (on general graphs). We combine the two tools into a recursive locality-based model checking algorithm. This algorithm is efficient on every monadically stable graph class admitting flip-closed sparse weak neighborhood covers, where flip-closure is a mild additional assumption. Thereby, establishing efficient first-order model checking on monadically stable classes is reduced to proving the existence of flip-closed sparse weak neighborhood covers on these classes - a purely combinatorial problem. We complete the picture by proving the existence of the desired covers for structurally nowhere dense classes: we show that every structurally nowhere dense class can be sparsified by contracting local sets of vertices, enabling us to lift the existence of covers from sparse classes.

==> chapters/outline.tex <==
\section{Technical Overview}


Assume we want to evaluate first-order sentences of quantifier rank $q$.
We will choose a radius $r$ as a function of $q$ and use the radius-$r$ Flipper game to build a recursive algorithm.
If the input graph $G$ is a winning position of Flipper then model checking is easy, since $G$ consists only of a single vertex.
We will assume we have a model checking algorithm for graphs where Flipper needs $d-1$ rounds to win
and show that we also have an algorithm for graphs where Flipper needs $d$ rounds to win.

So assume a graph $G$ with vertices $v_1,\dots,v_n$, where Flipper needs $d$ rounds to win the game.
At its core, our algorithm evaluates sentences of quantifier rank $q$ on $G$, 
using information gathered by evaluating sentences of quantifier rank $q$ on $r$-neighborhoods of $G$.
Each $r$-neighborhood $N_r[v_i]$ is a valid Flipper-move in the game and we can compute the responding flip $\flip F_i$ given by Flippers winning strategy.
The flipped $r$-neighborhoods $N_r[v_i] \oplus \flip F_i$ are now a positions where Flipper wins in $d-1$ rounds and thus
by induction we can efficiently evaluate sentences of quantifier rank $q$ on these graphs.
We can undo the flips within quantifier-free first-order logic, 
and thus we can even evaluate sentences of quantifier rank $q$ also on the original (unflipped) $r$-neighborhoods of $G$.

This lets us determine the $q$-types of neighborhoods of single vertices (called local $q$-types).
We show that two vertices with the same local $q$-type also have the same global $q$-type.
Thus, while we do not know the global $q$-types of the vertices in $G$, we at least know which vertices have the same $q$-type.
Since there are only finitely many $q$-types, we can build a representative set of vertices
and simplify the formula by ignoring all other vertices.
With some additional details described in Section ... this lets us evaluate formulas on $G$.

There is just one problem:
Assume the efficient algorithm for $d-1$-round graphs given by induction has a run time of, say, $O(n^{11})$ (with constant factors depending on $q$, $d$ and $\CC$).
Each $r$-neighborhood may have size up to $n$, and thus recursing into all $r$-neighborhoods leads to a run time of $\sum_{v \in V(G)} O(n^{11}) = O(n^{12})$.
Thus, with this naive approach, the degree of the polynomial increases by one for each round of the Flipper game.
This is bad, since depth of the Flipper game depends on $q$ and we aim for a run time, such as $O(n^{11})$, where the degree is independent of the input sentence.

This problem is fixed by neighborhood covers:
These are clusters $C_1,\dots,C_m$ of bounded radius $r'$ that contain all $r$-neighborhoods of the graph
such that each vertex is contained in $O(n^\eps)$ clusters for all $\eps > 0$.
This means $\sum_{1=1}^m |C_i| = O(n^{1+\eps})$.
We increase the radius of the Flipper game from $r$ to $r'$
and thus clusters are also valid Flipper-moves in the game.
We can hence evaluate sentences of quantifier rank $q$ on all clusters.
Since each $r$-neighborhood of the graph is contained in some cluster, this will give us sufficient information to evaluate sentences on $G$ itself.

Assume in depth $d-1$-graphs we have a run time of $O(n^{(1+\eps)^{d-1}} \cdot n^\stupidExponent)$ (with again constant factors depending in $q$, $d$ and $\CC$).
Then recursing into all clusters takes time $\sum_{i = 1}^m O(|C_i|^{(1+\eps)^{d-1}} \cdot n^\stupidExponent) =  O\bigl(\bigl(\sum_{i = 1}^m|C_i|\bigr)^{(1+\eps)^{d-1}} \cdot n^6\bigr) = O(n^{(1+\eps)^{d}} \cdot n^\stupidExponent)$.

Let $\Delta$ be the maximum number of rounds needed by the Flipper on graphs from $\CC$.
Since $\eps > 0$ can be chosen freely, we can set it for example to $1/\Delta$, leading (with $(1 + 1/\Delta)^\Delta \le e$) to a run time of 
$O(n^{6+e})$ for model checking on $\CC$.

==> covers-from-mmsc.tex <==
\begin{lemma}
    There is an algorithm that converts a
    fractional weak $r$-neighborhood cover with degree $d$ and spread $s$
    in time $O(n^2)$ into a weak $r$-neighborhood cover with degree $(d+2) \log(n)$ and spread $s$.
\end{lemma}

\begin{proof}
    Proofsketch:
    \begin{itemize}
        \item Let $\Chi$ be a fractional weak $r$-neighborhood cover with degree $d$ and spread $s$.
        \item We define the Minimum Membership Set Cover (MMSC) instance $(U,S)$ where 
        \begin{itemize}
            \item the universe $U = V(G) \times \{0,1\}$ contains for every vertex $v\in V(G)$ two copies $(v,1)$ and $(v,2)$
            \item the set system $S$ contains for every cluster $X \in \Chi$ a set $X$ containing for every $v\in V(G)$ the elements $(v,1)$ if $N(v) \subseteq X$ and $(v,2)$ if $v\in X$.
        \end{itemize}
        \item to prove: from $\Chi$ we can construct a solution with cost at most $d$ for the LP relaxation of the MMSC ILP for $(U,S)$.
        We therefore know that the LP relaxation has a solution with cost $z' \leq d$.
        \item We now want to apply the lemma from \cite{kuhn2005}, which reads as following.
        \begin{lemma}[Theorem 3 of \cite{kuhn2005}]
            For any MMSC instance, there exists a deterministic polynomial-time ap-
            proximation algorithm with an approximation ratio of $$(1 + O(1/\sqrt{z'}))(\log(|U|) + 1).$$
        \end{lemma}
        To apply it in our case we would need the following extended version of the statement:
        \begin{lemma}
            Given an MMSC instance $(U,S)$ \textcolor{blue}{whose LP relaxation has a solution with cost $z'$}, we can calculate an integer solution \textcolor{red}{in time $O((|U| + |S|)^c)$} with a cost of at most \textcolor{blue}{$(1 + O(1/\sqrt{z'})) \cdot (\log(|U|) + 1) \cdot z'$}.
        \end{lemma}

        Leaving us with the following TODOS:
\begin{itemize}
    \item \textcolor{blue}{We need to stress that the approximation factor is actually applied to the LP relaxation cost $z'$ and not the cost of an ILP solution.
    This should follow from the proof.}

\item         \textcolor{red}{We need to explicitly analyse the running time. Maybe cubic?}



\end{itemize}
        
\item We finally need to prove: every solution to $(U,S)$ with cost $z$ can be converted into a weak $r$-neighborhood cover with degree $z$ and spread $s$.

    \end{itemize}
\end{proof}


==> notation.tex <==
\section*{Notation}
\begin{itemize}
    \item Use american english over UK english
    \item Use the closed neighborhood $N_r[v] = \{u \in V(G) \mid \dist(u,v) \leq r\}$ to denote neighborhoods. Do \textbf{not} use the open neighborhood $N_r(v)$. Write $N_r[v] \setminus \{v\}$ if the open neighborhood is required.
    \item Quantifiers: use a $\sim$ space:
        \begin{itemize}
            \item $\exists x~\phi(\bar y)$
            \item $\exists x \in X~\phi(\bar y)$
        \end{itemize}
    \item Use \texttt{$\backslash$mid} to aggregate sets: 
    \begin{itemize}
        \item $\{p_i \mid i \in \N\}$
    \end{itemize}
    \item iffs, implications: use the \texttt{$\backslash$IFF}, \texttt{$\backslash$IMPLIES} command:
    \begin{itemize}
        \item $G \models \phi \IFF G \models \psi$
        \item $G \models \phi \IMPLIES G \models \psi$
    \end{itemize}
    \item The signature of formulas is implicit:
    \begin{itemize}
        \item a formula $\phi(\bar y)$ of quantifer rank at most $q$
    \end{itemize}
    \item Use neighborhoods instead of balls:
    \begin{itemize}
        \item $V_i$ is contained in an $r$-neighborhood of G
        \item when diameter is needed: $V_i$ contained in a subgraph of G with diameter at most $r$ 
    \end{itemize}
    \item Game radius: we don't use a global constant but define a constant $\rho = $ \texttt{$\backslash$mainRadius} in every lemma:
    \begin{itemize}
        \item Let $\rho = \mainRadius$ in...
    \end{itemize}


    \item Covers: we define them through flips and use spread instead of radius
    
    \item Capitalization: in headings, we capitalize every important word (the beginning, proper nouns, adjectives, ...)

    \item Write model checking instead of model-checking

    \item Write quantifier rank instead of quantifer-rank

    \item Write coat hanger and coat hanger free instead of coathanger
    
    \item We use $|G|$ instead of $|V(G)|$
    
    \item We use ``formula with quantifier rank $q$`` instead of ``formula of quantifier rank $q$``
    
    \item We use $X_i$ to denote clusters of a cover: $\{X_1,X_2,\ldots\}=\XX$ (Niko: that doesn't seem to work well for the guarding theorem, where we use $X$ as a color. Seb: Then we could use $C_i$ for clusters.)

    \item $\{u,v\}$ is an undirected edge and $(u,v)$ is a directed arc from $u$ to $v$. Use the word arc for directed edges. 
    \item Use $\varnothing$
    \item Use node for bush elements and vertex for graph elements.
    \item Nearly all American style guides recommend that both “i.e.” and “e.g.” be followed by a comma (this is also the case were you to write these abbreviations out as “that is” and “for example”).

\end{itemize}

\subsection*{To decide on:}
\begin{itemize}
    \item 
\end{itemize}


==> todos.tex <==

\listoftodos

